Dealing with Abbreviations in the Slovenian Biographical Lexicon

Abbreviations present a significant challenge for NLP systems because they cause tokenization and out-of-vocabulary errors. They can also make the text less readable, especially in reference printed books, where they are extensively used. Abbreviations are especially problematic in low-resource settings, where systems are less robust to begin with. In this paper, we propose a new method for addressing the problems caused by a high density of domain-specific abbreviations in a text. We apply this method to the case of a Slovenian biographical lexicon and evaluate it on a newly developed gold-standard dataset of 51 Slovenian biographies. Our abbreviation identification method performs significantly better than commonly used ad-hoc solutions, especially at identifying unseen abbreviations. We also propose and present the results of a method for expanding the identified abbreviations in context.

==> 1_introduction.tex <==
\section{Introduction}

Abbreviations such as "b." for "born", or "gr." for "graduated" are a common issue when dealing with digitized texts which use a large number of them for space-saving reasons.
They are also a known problem when processing technical documents \cite{park-byrd-2001-hybrid} and biomedical texts \cite{jin-etal-2019-deep-bio-abbr}. 
% and parliamentary transcriptions \cite{zelasko-2018-expanding}.
In this paper, we examine the case of biographical dictionaries, i.e.\ collections of biographies that have been digitized, and, in particular, the Slovenian Biographical Lexicon. 

To automatically extract facts from biographical texts, Digital Humanities researchers normally rely on out-of-the-box NLP tools such as Stanza \cite{qi-etal-2020-stanza} or SpaCy.\footnote{\url{https://spacy.io/}} These tools are often adequate for identifying sentences which are then used as input for higher-level downstream tasks, for manual inspection, and for visualization purposes. However, out-of-the-box tools are designed to work for the broadest possible text domains and cover the most common cases. This impacts performance significantly when dealing with domain-specific data, such as entries of biographical dictionaries, and more so when they contain a lot of abbreviations. The problem is even more pronounced when dealing with a relatively lower resource language, such as Slovenian. The performance bottleneck occurs already at the first step, i.e. tokenization: in order to perform good tokenization in domain-specific texts, we need to have a reliable method for identifying abbreviations such that the tokenizer does not split them wrongly, generating faulty tokens and incomplete sentences. In this paper we:


% Thus, they often fail to recognise, for example, abbreviations in domain-specific data such as entries in biographical dictionaries, especially if that data is in a relatively lower resource language, such as Slovenian. To perform successful tokenization in such conditions, we need a reliable method for identifying abbreviations to prevent the tokenizer from splitting them wrongly, generating faulty tokens and incomplete sentences. In this paper, we:
%ET: I don't understand the following sentence & is it really necessary?
%Likewise, in order to properly identify abbreviations, we need already an available tokenizer that generates clean training data. 
% On the other hand, nowadays one can use wordpiece tokenizers that arbitrarily split sequences of text into statistically meaningful token-pieces for the NLP task at hand. However,
 
%ET: I modified the following quite a lot, to be more in line with the standard intro to structure:
% The rest of the paper is structured as follows: in Section \ref{dataset} we introduce our dataset, in Section \ref{abbrev_impact} we quantify the impact that abbreviations have on a downstream task such as Named Entity Recognition (NER), in Section \ref{abbreviation_identif_expan} we then explain a novel method for dealing with abbreviations that does not rely on corpus-specific rules. We divide the task in two: first we train a system that takes raw text and returns a list of abbreviations that can be added as exceptions to tokenizers. Second, we mask each such abbreviation in the text and use the language model to predict the word that better fits in that context, which presumably is the expansion of the masked abbreviation. In Section \ref{evaluation} we measure the performance of both tasks on our test dataset. Section \ref{related_work} discussed related work, while Section \ref{conclusions} gives conclusions and directions for further work.

\begin{itemize}
    \setlength\itemsep{-0.5em}
    \item Quantify the effect that abbreviations have on a downstream task such as NER on Slovenian biographical texts. 
    \item Propose a method for abbreviation identification, apply it to raw texts and compare it to straightforward baselines.
    \item Analyze the feasibility of using contextually dependent word embeddings, in particular, the SloBERTa \cite{Ulcar_Sloberta:21} language model, to automatically expand abbreviations in text and improve readability.
    \item Evaluate the performance of our methods on a new human-curated dataset with, inter alia, gold tokens, sentences, named entities, and expanded abbreviations.\footnote{\url{https://github.com/angel-daza/abbreviation-detector}}
\end{itemize}


% We first analyze the impact of abbreviations on tokenization and sentence segmentation. We then compare the improvement achieved by two methods for abbreviation identification i) different count-based methods with a language dictionaries and ii) our proposed binary classifier based on SloBERTa \cite{Ulcar_Sloberta:21} that identifies each token as an abbreviation or not. Finally, we explore a method to substitute the abbreviations with their correct expansion in context using the masked predictions from SloBERTa and improve readability of the tokenized texts. 
% Once we identify the abbreviations, we can use this knowledge to improve the NLP pipelines by i) adding abbreviations to a lexicon and keeping the text as-is (i.e. we add the identified abbreviations as exceptions for the language-specific tokenizers) and ii) applying the high-confidence abbreviation expansions to substitute the abbreviations with the expanded tokens. The benefits of abbreviation expansion are not only for improving NLP performance, but also to improve the readability for researchers. Because many biographies contain an overwhelming amount of abbreviations, the clarity of the text sometimes obfuscates the meaning and lastly, our method addresses the problem of OOV abbreviations by avoiding the reliance on pre-made lexicons (which always will be incomplete) and bypasses the loophole of depending on pre-tokenized text for abbreviation identification. The goals of this paper are:
% , these standard tools suffer a big impact on performance. These mistakes are then carried to any downstream task that is applied when using these NLP pipelines.





==> 2_related_work.tex <==
\section{Related Work}\label{related_work}

Specific work addressing abbreviations is scarce. We think this is due to the fact that it is addressed as a preprocessing step with tailored solutions for each specific use case, involving regular expressions, or corpus-specific rules \cite{bollmann-etal-2011-rule}. A few papers try to construct methods for a general solution to this problem. For instance, \newcite{park-byrd-2001-hybrid} propose a pipeline system to induce acronyms, where every sequence of characters (separated by spaces) is considered a \textit{candidate abbreviation} if it satisfies certain conditions. \citet{zelasko-2018-expanding} proposes a more advanced approach based on an LSTM classifier that uses morphosyntactic information about a sentence to directly infer the correct expansion of an abbreviation in Polish. Direct work on abbreviations also exists in the biomedical domain, including detection and disambiguation \cite{stevenson-etal-2009-bio-abbr} as well as abbreviation expansion \cite{jin-etal-2019-deep-bio-abbr}. Finally, \citet{gorman-etal-2021-structured-abbreviation} have recently developed an English dataset to explore abbreviation expansion methods taking into account the context.

Another common way to address the difficulty of domain-specific texts is \textit{\textit{text normalization}}, which is the task of \textit{translating} a domain-specific text into more standard form (this can be at different levels such as lexical or morphological) that is easier to process by general purpose NLP tools. This approach is common when dealing with user generated text and social media \cite{pennell-liu-2011-character, baldwin-etal-2015-shared, van-der-goot-2019-monoise}, and also historical texts \cite{scherrer-erjavec-2013-modernizing, Ljubesic2016NormalisingSD, bollmann-2019-large}.

One drawback of text normalization is that it is frequently implemented using an Encoder-Decoder approach \cite{robertson-goldwater-2018-evaluating,bollmann-etal-2019-shot}, which requires a big-enough parallel corpus to be trained and obtain good-quality results. Another drawback is the fact that it \textit{generates} a new standard sentence, which is not a desired side effect if we want to preserve word by word the original biographical text. In contrast to the normalization task, we are interested in preserving the original text and only identifying (and perhaps expanding) the abbreviations that are problematic for the NLP tools.


==> 3_datasets.tex <==
\section{Dataset}\label{dataset}

%ET: it would be nice to put this in, if space allows:
%For space saving reasons the biographies contain many abbreviations, as illustrated in the following snippet, where %every fifth word is an abbreviation:
%
%\indent \textit{Agustich (Augustič) Imre, prekmurski pisatelj, r. 29. sept. 1837 v Murskih Petrovcih v Železni županiji, 
%u. v Budimpešti 17. jul. 1879. Šest gimn. razr. je dovršil v Sobotišču ...}



The Slovenian Biographical Lexicon (SBL) was published in 15 volumes (1925--1991) and contains 5,047 biographies \cite{sbl}. 
% It is fully digitised, encoded as a TEI document, and is available on the Web in the scope of the Slovenian Biography portal \cite{sbl}. 
For the experiments described in this paper, we have created the dataset SBL-51abbr \cite{11356/1588}, which consists of 51 randomly selected entries from SBL\footnote{\url{http://hdl.handle.net/11356/1588}}.
The text of each entry is manually tokenized and sentence segmented, marked with named entities, and lemmatized words. It has also been automatically annotated with Universal Dependencies PoS tags, morphological features and dependency parses using CLASSLA~\cite{ljubesic-dobrovoljc-2019-neural},\footnote{\url{https://pypi.org/project/classla/}} a fork of the Stanford Stanza pipeline \cite{qi-etal-2020-stanza},\footnote{\url{https://stanfordnlp.github.io/stanza/}} which is the state-of-the-art tool for annotating Slovenian. Crucially for the envisaged use of the corpus, the abbreviations in the corpus have been manually expanded so that the expansions are in the correct inflected form.
% given their sentence context.
The curated dataset consists of 655 sentences (see Table~\ref{tab:dataset_table}). It is available in the canonical TEI encoding, and derived plain text and CoNLL-U files. The plain-text file has abbreviations and their expansions marked up with [[...]]((...)) respectively. There are two CoNLL-U files, one with the text stream with abbreviations, and one with the text stream with expansions. Note that only the one with expansions has syntactic parses. Both CoNLL-U files have the expansions / abbreviations and named entities marked up in IOB format in the last column.

% and is available in several formats including the CoNLL-U format. 
% Information about the named entities and the abbreviations is given in the IOB format in the MISC (last) column. 
We use this dataset as a gold standard to test the performance of our proposed methods. We randomly split the available data into three portions: 70\% for training, 10\% for development and 20\% for testing. 

\begin{table}[htb]
\centering
\begin{tabular}{lrrrr}
Split              & Sents      & Abbrs   &  Unique  & Unseen \\\hline
Train              & 458        & 1385    &  399   & 0 \\
Dev                &  66        &  236    &  130   & 33 \\
Test               & 131        &  420    &  181   & 70 \\ \hline
$\Sigma$           & 655        & 2041    &  710   &
\end{tabular}
\caption{Abbreviation statistics on the SBL-51abbr dataset. We count the total number of abbreviations, the unique types and the number of unseen abbreviations in the dev and test splits.}
\label{tab:dataset_table}
\end{table}

==> 4_abbrev_impact.tex <==
\section{Impact of Abbreviations}\label{abbrev_impact}

We first quantify the impact that the high number of abbreviations in the SBL-51abbr corpus has when processing the raw texts with CLASSLA~\cite{ljubesic-dobrovoljc-2019-neural} and performing NER. We compare the performance on the original texts (with all abbreviations) with a second scenario where abbreviations were substituted with their gold expansions. Table~\ref{tab:NERvsNER} shows the performance per class when processing the original version (the first row of numbers per label), and right below is the performance when processing the same texts but without any abbreviation. There is a significant boost all across the board for the fully expanded texts, resulting on over 30 F1 points of improvement on the macro average measure. This shows that having effective methods for abbreviation identification and expansion can be beneficial.


\begin{table}[htb]
\centering
\begin{tabular}{ccccc}
\textbf{Label}              & \textbf{P} & \textbf{R} & \textbf{F1}    \\ \hline
\multirow{2}{*}{PER}        & 68.75      & 22.45      & 33.85        \\
                            & 76.80       & 65.31      & 70.59                    \\ \hline
\multirow{2}{*}{DERIV-PER}  & 50.00     & 4.76       & 8.70  \\
                            & 92.86      & 61.90       & 74.29             \\ \hline
\multirow{2}{*}{LOC}        & 85.29      & 39.73      & 54.21 \\
                            & 82.32      & 92.47      & 87.10    \\ \hline
\multirow{2}{*}{MISC}       & 65.38      & 12.41      & 20.86   \\
                            & 56.14      & 23.36      & 32.99          \\ \hline
\multirow{2}{*}{ORG}        & 23.53      & 14.81      & 18.18   \\
                            & 22.06      & 55.56      & 31.58            \\ \hline
\multirow{2}{*}{macro\_avg} & 58.59      & 18.83      & 27.16  \\
                            & 66.03      & 59.72      & 59.31     \\  \hline              
\end{tabular}
\caption{NER scores when applied to the original sentences with abbreviations (upper rows) vs sentences with all abbreviations expanded (lower rows).}
\label{tab:NERvsNER}
\end{table}

==> 5_abbrev_identif_expan.tex <==
\section{Dealing with Abbreviations}\label{abbreviation_identif_expan}

\begin{figure*}
\centering
  \includegraphics[width=0.85\textwidth]{EMNLP 2022/figs/SloBERTa2.png}
  \caption{We first train a classifier for identifying abbreviations (SloBERTa+Neural linear layer) and then match each of the identified candidates to use SloBERTa as a predictor for that slot. We only keep the suggested expansion if it meets the requirements.}
\label{fig:method}
\end{figure*}

\subsection{Baselines}

\textbf{Dictionary-based:} to bypass tokenizer-specific noise, we split every document by spaces to obtain a list of \textit{dirty tokens}.\footnote{We call them \textit{dirty} because they will have punctuation attached to them. For example "Hello world!" will be \textit{tokenized} as ['Hello', 'world!'] instead of ['Hello', 'world', '!'] which would be the optimal tokenization.} For each token, we first clean it, meaning we remove all special characters except full stops. If the \textit{clean token} does not end with a full stop we skip it, otherwise we strip the full stop and check if the entry exists in a large dictionary. We use two dictionaries: the Hunspell dictionary,\footnote{\url{https://github.com/hunspell/hunspell}} a popular tool used for spelling correction, and GigaFida 2.0 \cite{krek-etal-2020-gigafida}, a big reference corpus of standard Slovene. Because dictionaries only contain entries for complete words, we consider the token an abbreviation if no entry exists.

\textbf{Corpus-based:} we tokenize the training corpus using CLASSLA and compute the frequency for all token unigrams $t_1$ and bigrams $(t_1,t_2)$ in the corpus. If a bigram contains a full stop as a second component or if a unigram has a full stop as its last character,\footnote{We test for this case because, if the tokenizer rightly recognized the abbreviation, then the full stop will still be attached to it} then we increase the count of $t_1$ in $\mathcal{A}$ otherwise we increase the count of $t_1$ in $\mathcal{B}$. We take all $t_1$s that appear in both lists and calculate their probability to be an abbreviation as:

\begin{equation}
    P(t_1=abbr)=\frac{freq(t_1 \epsilon \mathcal{A})}{freq(t_1 \epsilon \mathcal{A})+freq(t_1 \epsilon \mathcal{B})}
\end{equation}

If the probability $P(t_1=abbr) \geq 0.8 $ then $t_1$ is considered to be an abbreviation, otherwise we skip it. This method will, of course, carry over some of the tokenization mistakes. The reasoning behind this baseline is to capture the number of times a given token appears before a full stop compared to the total times it appears in the corpus. If it is the case that most of the occurrences of such a token are immediately followed by a full stop, then it is most likely an (unrecognized) abbreviation.

\subsection{Abbreviation Classifier}
We propose an automatic method for identifying abbreviations by fine-tuning a classifier on top of the SLoBERTa language model \cite{Ulcar_Sloberta:21}. We again obtain the sequence of tokens by splitting the raw texts by spaces. We treat each one of the \textit{dirty tokens} as a separate input sequence to SloBERTa. We train the classifier using the gold abbreviation labels to predict if a token is an abbreviation or not (Figure \ref{fig:method}, bottom).

% \begin{figure}
% \centering
%   \includegraphics[width=0.5\textwidth]{figs/SloBERTa2.png}
%   \caption{We first train a classifier for identifying abbreviations (SloBERTa+Neural linear layer) and then mach each of the identified candidates to use SloBERTa as a predictor for that slot. We only keep the suggested expansion if it meets the requirements.}
% \label{fig:method}
% \end{figure}

\subsection{Abbreviation Expansion}
Once we have our text with abbreviation candidates identified, for each candidate, we take the full sentence it appears in, mask it and let SloBERTa predict the masked token. We take SloBERTa's prediction to be a valid expansion if one of the top~5 predicted candidates starts with the same letter as the masked abbreviation, otherwise we leave the original abbreviation. This way we are substituting each candidate \textit{in-context} and thus approaching the optimal scenario with the fully expanded sentences where NER performed much better (see Table~\ref{tab:NERvsNER}). A visualization of both the identification and expansion steps of our method is given in Figure~\ref{fig:method}.

==> 6_evaluation.tex <==
\section{Results and Evaluation}\label{evaluation}

\subsection{Abbreviation Identification Baselines}

We first present the results on the test set obtained by our proposed baselines in Table \ref{table:baselines}. These baselines represent common pre-processing approaches to dealing with abbreviations. We can see that the two dictionary versions suffer from low recall, especially the GigaFida dictionary with only 20\%. This behavior is expected since we are dealing with a domain-specific (and partially historical) text. The second baseline behaves much better and achieves an 85.34 F1 score. The Bigrams+Dict version mixes both approaches, which improves the coverage of identified abbreviations, but unfortunately lowers the high precision of the bigram approach.

\begin{table}[htb]
\centering
\begin{tabular}{lllll}
\textbf{Baseline}                & \textbf{P}     & \textbf{R}    &  \textbf{F1} \\ \hline
GigaFida Dict	        & 89.36	        & 20.00	    & 32.68 \\
Hunspell Dict	        & 80.81	        & 71.19	    & 75.70 \\
Corpus Bigrams	        & 95.85	        & 76.90	    & 85.34 \\
Bigrams+Dict	        & 73.27	        & 95.95	    & 83.09
\end{tabular}
\caption{Abbreviation identification baseline results on the test set. They show trade-offs between precision and recall. The bigrams method performs the best.}
\label{table:baselines}
\end{table}


\subsection{Abbreviation Classifier} 

The baselines show a trade-off between good precision or good recall. In contrast, Table \ref{table:sloberta} shows that our SloBERTa method significantly increases the recall without hampering precision. We fine-tuned SloBERTa\footnote{We used the default settings from HuggingFace \url{https://huggingface.co/EMBEDDIA/sloberta}} 
for 5 epochs and pick the model that performs best on the development set. We present the mean of 5 experiments with different random seeds together with the standard deviation. The results demonstrate that this is a stable approach for identifying abbreviations in text.

\begin{table}[htb]
\centering
\begin{tabular}{cccc}
\textbf{Split }  &  \textbf{P}     &    \textbf{R}            &   \textbf{F1}               \\\hline
Dev     &   95.91$^{\pm 0.75}$ 	   &    97.91$^{\pm 1.9}$ 	  &   96.89$^{\pm 0.9}$        \\
Test    &   $93.94^{\pm 1.5}$ 	   &    98.10$^{\pm 2.0}$     &   95.97$^{\pm 1.3}$        \\
\end{tabular}
\caption{Abbreviation identification results with our SloBERTa binary classifier. Results on test are 10 points above the best baseline.}\label{table:sloberta}
\end{table}

\subsection{Abbreviation Expansion} 
We measure the success of our abbreviation expansion method by re-running the NER tagger on the sentences with the expanded abbreviations as predicted by SloBERTa (see Table \ref{tab:NER_expanded}). From the 420 abbreviations in the test set, 154 where expanded following our heuristic and the rest of abbreviations in the sentences were left untouched. We can compare these scores directly with our analysis from Table~\ref{tab:NERvsNER} and see that even though our method for expanding is quite basic, it already gets us closer to the ceiling scores (where all gold expansions were substituted).  Important gains can be seen in all categories and the macro average score reached with the predicted expansions is 49.64 F1 which is 22 points above the 27.16 F1 obtained originally.

\begin{table}[htb]
\centering
\begin{tabular}{cccc}
\textbf{Label} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \hline
PER            & 40.54      & 67.67      & 50.70       \\
DERIV-PER      & 78.57      & 55.00      & 64.71       \\
LOC            & 72.33      & 82.73      & 77.18       \\
MISC           & 34.34      & 27.64      & 30.63       \\
ORG            & 17.14      & 46.15      & 25.00       \\\hline
macro\_avg     & 48.59      & 55.84      & 49.64      
\end{tabular}
\caption{The NER results on the test set after applying SloBERTa-based expansions show consistent improvements compared to the original sentences (cf. Table \ref{tab:NERvsNER})}
\label{tab:NER_expanded}
\end{table}

==> 7_conclusions.tex <==
\section{Conclusions}\label{conclusions}

In this paper we focused on the task of Named Entity Recognition to quantify the impact of abbreviations in a text by comparing the performance of the CLASSLA NER tagger on the same sentences with and without abbreviations. We presented a gold-standard dataset consisting of 51 biographies in Slovenian (a limited-resource language) in a specialized text domain. We also presented a method for automatically identifying abbreviations and expanding them without the need for a tokenizer. The biggest advantage of our method is that it can be applied out-of-the-box for any language which has a large language model available and does not need ad-hoc training data or large fixed dictionaries. Our abbreviation identification classifier obtains better precision and better recall when compared to other straightforward approaches to identify abbreviations. 

Finally, we presented a method that uses a pre-trained language model to predict plausible expansions for the identified abbreviations. We notice that our method is still simple but already achieves better results than directly processing the original sentences with abbreviations. In future work we aim to explore more sophisticated methods for abbreviation expansion that allow us to further improve the readability of texts. We find our results encouraging for researchers working with limited domains who may find a similar approach helpful for improving performance in other tasks.

% Even though our expansion method is far from ideal, the fact that the abbreviation classifier has such good results, allows us to e.g. add the abbreviations as exceptions to the tokenizers.

==> EMNLP 2022/related_work_long.tex <==
\section{Related Work}

\subsection{A raw draft of related work section including more sources}

\textbf{Abbreviations in NLP.}
Specific work addressing abbreviations is scarce. We think this is due to the fact that it is addressed as a preprocessing step with tailored solutions for each specific use case, frequently involving regular expressions, or corpus-specific rules \cite{bollmann-etal-2011-rule}. A few works try to construct methods for a general solution to this problem. For instance, \cite{park-byrd-2001-hybrid} propose a pipeline system to induce acronyms, where every sequence of characters (separated by spaces) is considered a \textit{candidate abbreviation} if it satisfies certain conditions

A common way to address the difficulty of domain-specific texts is \textit{\textit{text normalization}}, which is the task of \textit{translating} a domain-specific text into more standard form (this can be at different levels such as lexical or morphological) that is easier to process by general purpose NLP tools. This approach is common when dealing with user generated text and social media \cite{pennell-liu-2011-character, baldwin-etal-2015-shared, van-der-goot-2019-monoise}, and also historical texts \cite{scherrer-erjavec-2013-modernizing, Ljubesic2016NormalisingSD, bollmann-2019-large}.

One drawback of text normalization is that it is frequently implemented using an Encoder-Decoder approach \cite{robertson-goldwater-2018-evaluating,bollmann-etal-2019-shot}, which requires a big-enough parallel corpus to be trained and obtain good-quality results. Another drawback is the fact that it \textit{generates} a new standard sentence, which is not a desired side effect if we want to preserve word by word the original biographical text. In contrast to the normalization task, we are interested in preserving the original text and only identifying (and perhaps expanding) the abbreviations that are problematic for the NLP tools. Finally, it is also worth mentioning a similar concurrent work to ours \cite{gorman-etal-2021-structured-abbreviation} who work on expanding abbreviations in context for English texts.


One such method is from [Park, 2001] who propose a pipeline system to induce acronyms\footnote{In this work they address particularly the acronym types of abbreviations} from their definitions. The system has 5 components: abbreviation recognizer, definition finder, rule applier, abbreviation matcher and best match selector. It assumes that the beginning of a document contains the definition of an abbreviation, i.e. when it is first introduced for the reader, and tries to exploit this to obtain the definitions if the same acronym appears later in the document.

A string of alphabetic, numeric and special characters is considered as a \textit{candidate abbreviation} if it satisfies the following three conditions: i) its first character is alphabetic or numeric, ii) its length is between 2 and 10 characters, iii) it contains at least 1 capital letter, as well as three restrictions: i) It is not a known (dictionary) word, and is not the first word in a sentence, ii) it is not a predefined Person or Location and iii) it is not a member of a user defined list of stopwords.

They test their pipeline with three domain-specific documents (an automotive engineering book, a technical book from a pharmaceutical company, and NASA press releases for 1999.) and find that it works with more than 90\% accuracy, however this is for the specific case of documents which could be manually double checked and that follow the expected pattern of containing their definitions inside the same document. On the other hand, we are interested in abbreviations in general (not only acronyms) and we also aim to expand them in thousands of documents and have a more complicated case of abbreviations in context.

[Zelasko, 2018] try to use the morphosyntactic information of a sentence to infer the correct expansion of an abbreviation in Polish, a highly inflected language, which is closer to the cases we are aiming to solve\footnote{For example in Polish, the abbreviation "r." could be expanded into one of {rok, roku, rokowi, rokiem}, all of which mean "year" in English, but are inflected differently, based on the context in which they are used. [CITE Zelasko again]}. They use a Bidirectional LSTM that processes a sequence of morphosyntactic tag embeddings (1-1 correspondence with the words in a sentence), and a special tag for the abbreviation that tells the network which is the slot to be predicted. The LSTM predicts the morph. tag of the SLOT). The correctly inflected abbreviation expansion is obtained by a lookup of the base form and predicted morphological tag in a morphological dictionary. We are different because we don't aim to use any explicit morphological information, instead we will use a big LM to directly induce the inflected form in-context.

[Pennell 2011] use a character MT system to learn mappings between character-level “phrases” to be robust to new abbreviations, and an in-domain language model to learn the context of neighboring words. They build a compound score which takes into account word count index, perplexity in the in-domain LM, OOV counts and relative frequencies in the corpus. Using this score they chose the expansion hypothesis that is better ranked. This system is closer to ours in the sense that it uses the information of a LM to predict an expansion. we aim to exploit the existence of big LM and we don't need a compound corpus-dependent score to predict our abbreviations.

\textbf{Normalization of Historical Texts.}
A more general task related to ours is the normalization of historical texts, which is the task of mapping historical word forms to their modern counterparts.

To increase the effectivity of standard NLP tools, one line of work aims to \textit{normalize} historical text into standard text, where archaisms or source specific patterns should be translated into the modern standardized language. 

Normalization pre-suposes the existence of parallel corpora and need word-alignments

Works derived on word-alignment and character based SMT models:


[Bollman 2011] use a word-aligned old and a modern bible to induce a set of rules that can be used to \textit{translate} early new high german (16th century) to modern german lexica.

[Scherrer and Erjavec 2013] used lexicon of modern slovenian to find equivalent expressions in historic texts using character-based SMT...

[Ljubesic 2016] extend [Scherrer 2013] to test several variants of character-based SMT to normalise the spelling of their words (a token-token translation and a phrase-based translation). They use the Reference corpus of historical Slovene (goo300k) [CITE] which is was manually annotated for its normalised (modernised) word form(s), their part-of-speech, lemma, and — for archaic words — its gloss, i.e. contemporary synonym... Instead of using a lexicon, they use Giza++ to word-align the historic version to the modernized version and KENLM as a target slovenian language model to train their system.

Works with ML or DL:
[Korchagina 2017] compares rule-based, statistical machine translation, and neural machine translation for normalizing 16th century german into modern german. She finds that character-NMT is the best for her case

[Bollman 2019] A Large-Scale Comparison of Historical Text Normalization Systems

[Makarov 2020]  use generative modeling and expectation–maximization to normalize texts in a semi-supervised manner, avoiding the need of large manually normalized parallel datasets.


\subsection{Normalization of Historical Texts}

\textbf{Normalizing Medieval German Texts: from rules to deep learning} [Korchagina 2017]
        - Compares three methods: edit-based, statistical MT and neural MT
        - The baseline data is a manually normalized subset of the
        corpus, 2500 historical-modern word pairs (German 1450-1550 —> German). This was augmented with other databases available to assess the impact of training data size on the results.
        - Character Enc-Dec approach gave the best results with sentence-aligned training data > 20,000 pairs. Almost 8 points above the rule-based-distance methods
        
\textbf{Normalising Slovene data: historical texts vs. user-generated content.} [Ljubesic 2016] This work uses Char-based SMT to normalize text. This paper is very valuable for evaluaton setup! Distinguish between normalization and modernization:
        
Sanchez-Martines (2013) bootstrapped historical to modern lexica without word alignments
        
Scherrer and Erjavec (2013) used lexicon of modern slovenian to find *equivalent* expressions in historic texts
        
\textbf{Few-Shot and Zero-Shot Learning for Historical Text Normalization}

\textbf{Evaluating historical text normalization systems: How well do they generalize?}
    
\textbf{Rule-Based Normalization of Historical Texts} [Bollman, 2011]
    
\textbf{A Large-Scale Comparison of Historical Text Normalization Systems} [Bollman, 2019]
    
\textbf{Learning attention for historical text normalization by learning to pronounce}
    
\textbf{Semi-supervised Contextual Historical Text Normalization} [Makarov 2020]

\subsection{Work on Abbreviations}

\textbf{Hybrid text mining for finding abbreviations and their definitions} [Park, 2001]
    
    This system has **5 components**: abbreviation recognizer, definition finder, rule
    applier, abbreviation matcher and best match selector
    
    It assumes that the beginning of a document contains the definition of an abbreviation, i.e. when it is first introduced for the reader, and tries to exploit this to obtain the definitions.
    
    They consider a string of alphabetic, numeric and special characters as a
    **candidate abbreviation** if it satisfies the following three conditions: 
    
    1. Its first character is alphabetic or numeric
    2. Its length is between 2 and 10 characters
    3. It contains at least 1 capital letter
    
    and three restrictions:
    
    1. It is not a known (dictionary) word, and is not the first word in a sentence 
    2. It is not a predefined Person or Location 
    3. It is not a member of user defined stopwords
    
\textbf{Expanding Abbreviations in a Strongly Inflected Language: Are Morphosyntactic Tags Sufficient?} [Zelasko, 2018]
    
    They try to use the morphosyntactic information of a sentence to infer the correct expansion of an abbreviation. They use a Bidirectional LSTM that process the sequence of morphosyntactic tag embeddings (1-1 correspondence with the words in a sentence), a special tag for the abbreviation which tells the network that that is the slot to be predicted (it predicts the morph. tag of the SLOT). The correctly inflected abbreviation expansion is obtained by a lookup of the base form and predicted morphological tag in a morphological dictionary.
    
    For example in Polish, the abbreviation "r." could be expanded into one of {rok, roku, rokowi, rokiem}, all of which mean "year" in English, but are inflected differently, based on the context in which they are used.
    
    Select 34 Polish words which are often abbreviated 4.1., look up their inflected forms in the Polimorf morphological dictionary. They get 84% abbr. prediction accuracy in training set and 74% in test set.
    
\textbf{A Character-Level Machine Translation Approach for Normalization of SMS Abbreviations }[Pennell 2011]
    
    > An annotator’s time is wasted if he is presented with many messages containing no abbreviations, or with sentences all containing the same, very common abbreviations.
    > 
    - A scoring system was thus devised using the following metrics:
        - **Word-Count Index:** shows is a message is shorter than average
        - **Char-LM Perplexity Scores:** eliminate the cases with too much perplexity (gibberish)
        - **OOV Counts:** how many words in a sentence are OOV. Skip OOV=0 since they are "too common"
        - **OOV Percentages:** s1 = OOV words / N and s2 = Unique-OOV / Unique-N. If s1 > 0.5 but s2 is not then the example is ignored
        - **Global OOV Freq:** to ensure that a representative abbreviation is being substituted
    
    > A sorted list is generated for each metric. The final score for each sentence is a weighted average of its position in each list, with more weight given to the non-duplicate OOV percentage and less weight given to the OOV frequency scores.
    > 
    
    Uses  a two-phase approach for SMS normalization. The **first phase uses a character-level** MT system to generate possible hypotheses for each abbreviation. The **second uses a word-level language model (LM)** to choose a hypothesis in context.
    

\textbf{Disambiguation of Biomedical Abbreviations} [Stevenson, 2009]

\textbf{Deep Contextualized Biomedical Abbreviation Expansion} [Jin, 2019]

==> EMNLP 2022/related_work_old.tex <==

\section{Related Work}\label{related_work}

Abbreviations are normally handled at the pre-processing steps, with regular expressions and pattern matching. For instance, \citet{park-byrd-2001-hybrid} propose a pipeline system to induce acronyms, where every sequence of characters (separated by spaces) is considered a \textit{candidate abbreviation} if it satisfies certain conditions. \citet{zelasko-2018-expanding} propose a more advanced approach based on an LSTM classifier that uses morphosyntactic information about a sentence to directly infer the correct expansion of an abbreviation in Polish. 

Another related task is text normalization, which is the task of translating a domain-specific text into a standard form that is easier to process by NLP tools \cite{Ljubesic2016NormalisingSD,bollmann-etal-2019-shot}. The drawback of text normalization is that it is normally implemented using an Encoder-Decoder approach \cite{bollmann-2019-large}, which requires a big-enough parallel corpus to obtain satisfying results.



==> related_work_long.tex <==
\section{Related Work}

\subsection{A raw draft of related work section including more sources}

\textbf{Abbreviations in NLP.}
Specific work addressing abbreviations is scarce. We think this is due to the fact that it is addressed as a preprocessing step with tailored solutions for each specific use case, frequently involving regular expressions, or corpus-specific rules \cite{bollmann-etal-2011-rule}. A few works try to construct methods for a general solution to this problem. For instance, \cite{park-byrd-2001-hybrid} propose a pipeline system to induce acronyms, where every sequence of characters (separated by spaces) is considered a \textit{candidate abbreviation} if it satisfies certain conditions

A common way to address the difficulty of domain-specific texts is \textit{\textit{text normalization}}, which is the task of \textit{translating} a domain-specific text into more standard form (this can be at different levels such as lexical or morphological) that is easier to process by general purpose NLP tools. This approach is common when dealing with user generated text and social media \cite{pennell-liu-2011-character, baldwin-etal-2015-shared, van-der-goot-2019-monoise}, and also historical texts \cite{scherrer-erjavec-2013-modernizing, Ljubesic2016NormalisingSD, bollmann-2019-large}.

One drawback of text normalization is that it is frequently implemented using an Encoder-Decoder approach \cite{robertson-goldwater-2018-evaluating,bollmann-etal-2019-shot}, which requires a big-enough parallel corpus to be trained and obtain good-quality results. Another drawback is the fact that it \textit{generates} a new standard sentence, which is not a desired side effect if we want to preserve word by word the original biographical text. In contrast to the normalization task, we are interested in preserving the original text and only identifying (and perhaps expanding) the abbreviations that are problematic for the NLP tools. Finally, it is also worth mentioning a similar concurrent work to ours \cite{gorman-etal-2021-structured-abbreviation} who work on expanding abbreviations in context for English texts.


One such method is from [Park, 2001] who propose a pipeline system to induce acronyms\footnote{In this work they address particularly the acronym types of abbreviations} from their definitions. The system has 5 components: abbreviation recognizer, definition finder, rule applier, abbreviation matcher and best match selector. It assumes that the beginning of a document contains the definition of an abbreviation, i.e. when it is first introduced for the reader, and tries to exploit this to obtain the definitions if the same acronym appears later in the document.

A string of alphabetic, numeric and special characters is considered as a \textit{candidate abbreviation} if it satisfies the following three conditions: i) its first character is alphabetic or numeric, ii) its length is between 2 and 10 characters, iii) it contains at least 1 capital letter, as well as three restrictions: i) It is not a known (dictionary) word, and is not the first word in a sentence, ii) it is not a predefined Person or Location and iii) it is not a member of a user defined list of stopwords.

They test their pipeline with three domain-specific documents (an automotive engineering book, a technical book from a pharmaceutical company, and NASA press releases for 1999.) and find that it works with more than 90\% accuracy, however this is for the specific case of documents which could be manually double checked and that follow the expected pattern of containing their definitions inside the same document. On the other hand, we are interested in abbreviations in general (not only acronyms) and we also aim to expand them in thousands of documents and have a more complicated case of abbreviations in context.

[Zelasko, 2018] try to use the morphosyntactic information of a sentence to infer the correct expansion of an abbreviation in Polish, a highly inflected language, which is closer to the cases we are aiming to solve\footnote{For example in Polish, the abbreviation "r." could be expanded into one of {rok, roku, rokowi, rokiem}, all of which mean "year" in English, but are inflected differently, based on the context in which they are used. [CITE Zelasko again]}. They use a Bidirectional LSTM that processes a sequence of morphosyntactic tag embeddings (1-1 correspondence with the words in a sentence), and a special tag for the abbreviation that tells the network which is the slot to be predicted. The LSTM predicts the morph. tag of the SLOT). The correctly inflected abbreviation expansion is obtained by a lookup of the base form and predicted morphological tag in a morphological dictionary. We are different because we don't aim to use any explicit morphological information, instead we will use a big LM to directly induce the inflected form in-context.

[Pennell 2011] use a character MT system to learn mappings between character-level “phrases” to be robust to new abbreviations, and an in-domain language model to learn the context of neighboring words. They build a compound score which takes into account word count index, perplexity in the in-domain LM, OOV counts and relative frequencies in the corpus. Using this score they chose the expansion hypothesis that is better ranked. This system is closer to ours in the sense that it uses the information of a LM to predict an expansion. we aim to exploit the existence of big LM and we don't need a compound corpus-dependent score to predict our abbreviations.

\textbf{Normalization of Historical Texts.}
A more general task related to ours is the normalization of historical texts, which is the task of mapping historical word forms to their modern counterparts.

To increase the effectivity of standard NLP tools, one line of work aims to \textit{normalize} historical text into standard text, where archaisms or source specific patterns should be translated into the modern standardized language. 

Normalization pre-suposes the existence of parallel corpora and need word-alignments

Works derived on word-alignment and character based SMT models:


[Bollman 2011] use a word-aligned old and a modern bible to induce a set of rules that can be used to \textit{translate} early new high german (16th century) to modern german lexica.

[Scherrer and Erjavec 2013] used lexicon of modern slovenian to find equivalent expressions in historic texts using character-based SMT...

[Ljubesic 2016] extend [Scherrer 2013] to test several variants of character-based SMT to normalise the spelling of their words (a token-token translation and a phrase-based translation). They use the Reference corpus of historical Slovene (goo300k) [CITE] which is was manually annotated for its normalised (modernised) word form(s), their part-of-speech, lemma, and — for archaic words — its gloss, i.e. contemporary synonym... Instead of using a lexicon, they use Giza++ to word-align the historic version to the modernized version and KENLM as a target slovenian language model to train their system.

Works with ML or DL:
[Korchagina 2017] compares rule-based, statistical machine translation, and neural machine translation for normalizing 16th century german into modern german. She finds that character-NMT is the best for her case

[Bollman 2019] A Large-Scale Comparison of Historical Text Normalization Systems

[Makarov 2020]  use generative modeling and expectation–maximization to normalize texts in a semi-supervised manner, avoiding the need of large manually normalized parallel datasets.


\subsection{Normalization of Historical Texts}

\textbf{Normalizing Medieval German Texts: from rules to deep learning} [Korchagina 2017]
        - Compares three methods: edit-based, statistical MT and neural MT
        - The baseline data is a manually normalized subset of the
        corpus, 2500 historical-modern word pairs (German 1450-1550 —> German). This was augmented with other databases available to assess the impact of training data size on the results.
        - Character Enc-Dec approach gave the best results with sentence-aligned training data > 20,000 pairs. Almost 8 points above the rule-based-distance methods
        
\textbf{Normalising Slovene data: historical texts vs. user-generated content.} [Ljubesic 2016] This work uses Char-based SMT to normalize text. This paper is very valuable for evaluaton setup! Distinguish between normalization and modernization:
        
Sanchez-Martines (2013) bootstrapped historical to modern lexica without word alignments
        
Scherrer and Erjavec (2013) used lexicon of modern slovenian to find *equivalent* expressions in historic texts
        
\textbf{Few-Shot and Zero-Shot Learning for Historical Text Normalization}

\textbf{Evaluating historical text normalization systems: How well do they generalize?}
    
\textbf{Rule-Based Normalization of Historical Texts} [Bollman, 2011]
    
\textbf{A Large-Scale Comparison of Historical Text Normalization Systems} [Bollman, 2019]
    
\textbf{Learning attention for historical text normalization by learning to pronounce}
    
\textbf{Semi-supervised Contextual Historical Text Normalization} [Makarov 2020]

\subsection{Work on Abbreviations}

\textbf{Hybrid text mining for finding abbreviations and their definitions} [Park, 2001]
    
    This system has **5 components**: abbreviation recognizer, definition finder, rule
    applier, abbreviation matcher and best match selector
    
    It assumes that the beginning of a document contains the definition of an abbreviation, i.e. when it is first introduced for the reader, and tries to exploit this to obtain the definitions.
    
    They consider a string of alphabetic, numeric and special characters as a
    **candidate abbreviation** if it satisfies the following three conditions: 
    
    1. Its first character is alphabetic or numeric
    2. Its length is between 2 and 10 characters
    3. It contains at least 1 capital letter
    
    and three restrictions:
    
    1. It is not a known (dictionary) word, and is not the first word in a sentence 
    2. It is not a predefined Person or Location 
    3. It is not a member of user defined stopwords
    
\textbf{Expanding Abbreviations in a Strongly Inflected Language: Are Morphosyntactic Tags Sufficient?} [Zelasko, 2018]
    
    They try to use the morphosyntactic information of a sentence to infer the correct expansion of an abbreviation. They use a Bidirectional LSTM that process the sequence of morphosyntactic tag embeddings (1-1 correspondence with the words in a sentence), a special tag for the abbreviation which tells the network that that is the slot to be predicted (it predicts the morph. tag of the SLOT). The correctly inflected abbreviation expansion is obtained by a lookup of the base form and predicted morphological tag in a morphological dictionary.
    
    For example in Polish, the abbreviation "r." could be expanded into one of {rok, roku, rokowi, rokiem}, all of which mean "year" in English, but are inflected differently, based on the context in which they are used.
    
    Select 34 Polish words which are often abbreviated 4.1., look up their inflected forms in the Polimorf morphological dictionary. They get 84% abbr. prediction accuracy in training set and 74% in test set.
    
\textbf{A Character-Level Machine Translation Approach for Normalization of SMS Abbreviations }[Pennell 2011]
    
    > An annotator’s time is wasted if he is presented with many messages containing no abbreviations, or with sentences all containing the same, very common abbreviations.
    > 
    - A scoring system was thus devised using the following metrics:
        - **Word-Count Index:** shows is a message is shorter than average
        - **Char-LM Perplexity Scores:** eliminate the cases with too much perplexity (gibberish)
        - **OOV Counts:** how many words in a sentence are OOV. Skip OOV=0 since they are "too common"
        - **OOV Percentages:** s1 = OOV words / N and s2 = Unique-OOV / Unique-N. If s1 > 0.5 but s2 is not then the example is ignored
        - **Global OOV Freq:** to ensure that a representative abbreviation is being substituted
    
    > A sorted list is generated for each metric. The final score for each sentence is a weighted average of its position in each list, with more weight given to the non-duplicate OOV percentage and less weight given to the OOV frequency scores.
    > 
    
    Uses  a two-phase approach for SMS normalization. The **first phase uses a character-level** MT system to generate possible hypotheses for each abbreviation. The **second uses a word-level language model (LM)** to choose a hypothesis in context.
    

\textbf{Disambiguation of Biomedical Abbreviations} [Stevenson, 2009]

\textbf{Deep Contextualized Biomedical Abbreviation Expansion} [Jin, 2019]

==> related_work_old.tex <==

\section{Related Work}\label{related_work}

Abbreviations are normally handled at the pre-processing steps, with regular expressions and pattern matching. For instance, \citet{park-byrd-2001-hybrid} propose a pipeline system to induce acronyms, where every sequence of characters (separated by spaces) is considered a \textit{candidate abbreviation} if it satisfies certain conditions. \citet{zelasko-2018-expanding} propose a more advanced approach based on an LSTM classifier that uses morphosyntactic information about a sentence to directly infer the correct expansion of an abbreviation in Polish. 

Another related task is text normalization, which is the task of translating a domain-specific text into a standard form that is easier to process by NLP tools \cite{Ljubesic2016NormalisingSD,bollmann-etal-2019-shot}. The drawback of text normalization is that it is normally implemented using an Encoder-Decoder approach \cite{bollmann-2019-large}, which requires a big-enough parallel corpus to obtain satisfying results.


